Improving 3D Pose Estimation for Sign Language

This work addresses 3D human pose reconstruction in single images. We present a method that combines Forward Kinematics (FK) with neural networks to ensure a fast and valid prediction of 3D pose. Pose is represented as a hierarchical tree/graph with nodes corresponding to human joints that model their physical limits. Given a 2D detection of keypoints in the image, we lift the skeleton to 3D using neural networks to predict both the joint rotations and bone lengths. These predictions are then combined with skeletal constraints using an FK layer implemented as a network layer in PyTorch. The result is a fast and accurate approach to the estimation of 3D skeletal pose. Through quantitative and qualitative evaluation, we demonstrate the method is significantly more accurate than MediaPipe in terms of both per joint positional error and visual appearance. Furthermore, we demonstrate generalization over different datasets. The implementation in PyTorch runs at between 100-200 milliseconds per image (including CNN detection) using CPU only.

==> tables/table_human36.tex <==
% \begin{table*}[ht]
% \centering
% \setlength{\tabcolsep}{3.3pt}
% \begin{tabular}{@{}lrrrrrrrrrrrrrrrr@{}}\toprule
% \multicolumn{1}{c}{Protocol \#1} & \multicolumn{16}{c}{Mean Per Joint Position Error (mm) per sequence and average} \\\hline

% \multicolumn{1}{c|}{Competitors:} & \multicolumn{1}{c|}{Direct.} & \multicolumn{1}{c|}{Discuss.}  & \multicolumn{1}{c|}{Eating} & \multicolumn{1}{c|}{Greet} & \multicolumn{1}{c|}{Phone} & \multicolumn{1}{c|}{Photo} & \multicolumn{1}{c|}{Pose} & \multicolumn{1}{c|}{Purch.} & \multicolumn{1}{c|}{Sitting} & \multicolumn{1}{c|}{Sit.D.} & \multicolumn{1}{c|}{Smoke} & \multicolumn{1}{c|}{Wait} & \multicolumn{1}{c|}{WalkD} & \multicolumn{1}{c|}{Walk} & \multicolumn{1}{c|}{WalkT.} & \multicolumn{1}{c}{{\bf Avg.}}
% \\ \hline
% Ionescu~{\etal}~\cite{journals/pami/IonescuPOS14} & 132.7 & 183.6 & 132.3 & 164.4 & 162.1 & 205.9 & 150.6 & 171.3 & 151.6 & 243.0 & 162.1 & 170.7 & 177.1 & 96.6 & 127.9 & 162.1\\
% Tekin~{\etal}~\cite{tekin_2016_direct} & 102.4 & 147.2 & 88.8 & 125.3 & 118.0 & 182.7 & 112.4 & 129.2 & 138.9 & 224.9 & 118.4 & 138.8 & 126.3 & 55.1 & 65.8 & 125.0\\
% Zhou~{\etal}~\cite{zhou_2016_sparseness} & 87.4 & 109.3 & 87.1 & 103.2 & 116.2 & 143.3 & 106.9 & 99.8 & 124.5 & 199.2 & 107.4 & 118.1 & 114.2 & 79.4 & 97.7 & 113.0\\
% Du~{\etal}~\cite{Du_markerless} & 85.1 & 112.7 & 104.9 & 122.1 & 139.1 & 135.9 & 105.9 & 166.2 & 117.5 & 226.9 & 120.0 & 117.7 & 137.4 & 99.3 & 106.5 & 126.5\\
% Chen~{\etal}~\cite{chen_3d_human_2017} & 89.9 & 97.6 & 89.9 & 107.9 & 107.3 & 139.2 & 93.6 & 136.0 & 133.1 & 240.1 & 106.6 & 106.2 & 87.0 & 114.0 & 90.5 & 114.1\\
% Pavlakos~{\etal}~\cite{Pavlakos2017CoarsetoFineVP} & 67.4 & 71.9 & 66.7 & 69.1 & 72.0 & 77.0 & 65.0 & 68.3 & 83.7 & 96.5 & 71.7 & 65.8 & 74.9 & 59.1 & 63.2 & 71.9\\
% Mehta~{\etal}~\cite{mehta_2017_in_wild} & 52.6 & 64.1 & 55.2 & 62.2 & 71.6 & 79.5 & 52.8 & 68.6 & 91.8 & 118.4 & 65.7 & 63.5 & 49.4 & 76.4 & 53.5 & 68.6\\
% Zhou~{\etal}~\cite{Zhou_2017_ICCV} & 54.8 & 60.7 & 58.2 & 71.4 & 62.0 & 65.5 & 53.8 & 55.6 & 75.2 & 111.6 & 64.1 & 66.0 & 51.4 & 63.2 & 55.3 & 64.9\\
% Martinez~{\etal}~\cite{martinez_2017_3dbaseline} & 51.8 & 56.2 & 58.1 & 59.0 & 69.5 & 78.4 & 55.2 & 58.1 & 74.0 & 94.6 & 62.3 & 59.1 & 65.1 & 49.5 & 52.4 & 62.9\\
% Sun~{\etal}~\cite{sun_2017_compositional} & 52.8 & 54.8 & 54.2 & 54.3 & 61.8 & 53.1 & 53.6 & 71.7 & 86.7 & 61.5 & 67.2 & 53.4 & 47.1 & 61.6 & 53.4 & 59.1\\
% Fang~{\etal}~\cite{Fang2018LearningPG} & 50.1 & 54.3 & 57.0 & 57.1 & 66.6 & 73.3 & 53.4 & 55.7 & 72.8 & 88.6 & 60.3 & 57.7 & 62.7 & 47.5 & 50.6 & 60.4\\
% Yang~{\etal}~\cite{Yang20183DHP} & 51.5 & 58.9 & 50.4 & 57.0 & 62.1 & 65.4 & 49.8 & 52.7 & 69.2 & 85.2 & 57.4 & 58.4 & 43.6 & 60.1 & 47.7 & 58.6\\
% Hossain~{\etal}~\cite{Hossain_exploiting_2018} & 48.4 & 50.7 & 57.2 & 55.2 & 63.1 & 72.6 & 53.0 & 51.7 & 66.1 & 80.9 & 59.0 & 57.3 & 62.4 & 46.6 & 49.6 & 58.3\\
% Zhao~{\etal}~\cite{zhaoCVPR19semantic} & 47.3 & 60.7 & 51.4 & 60.5 & 61.1 & 49.9 & 47.3 & 68.1 & 86.2 & 55.0 & 67.8 & 61.0 & 42.1 & 60.6 & 45.3 & 57.6\\
% Li~{\etal}~\cite{li2020hybrik} & -& -& -& -& -& -& -& -& -& -& -& -& -& -& -& 54.4\\
% Wandt~{\etal}~\cite{elepose} & -& -& -& -& -& -& -& -& -& -& -& -& -& -& -& 64.0\\\toprule
% Proposed & 60.9 & 67.6 & 62.7 & 65.5 & 77.8 & 84.7 & 61.0 & 74.4 & 86.2 & 97.8 & 72.1 & 67.1 & 74.4 & 53.8 & 58.4 & 71.0
% \\\toprule
% \end{tabular}
% \caption{The evaluation comparison of the proposal method and competitors (sorted in chronological order).
% Results report MPJPE error (mm) per column for each individual sequence motion ({\eg} Sitting) of \textsc{Human3.6M} dataset.
% The evaluation configuration is protocol \#1 that takes subjects S1, S5, S6, S7, and S8 for training, and S9 and S11 for testing.
% The lowest error (per column) is highlighted in bold, and the last column ({\bf Avg.}) shows the average over all sequences per method.
% This table was partly imported from~\cite{zhaoCVPR19semantic}.
% }
% \label{table:human36_big}
% \end{table*}
% % np.mean([float(y) for y in ''.split(' ')])

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[ht]
% \centering
% \caption{Average, median, and standard deviation per joint position errors (cm) on test subjects (S9 and S11) for~\textsc{Human3.6M}.
% Individual rows show a specific alignment.% ($\mathcal{B}$ -- GT bones lengths, $\mathbf{R}$ -- Kabsch-Umeyama rotational alignment, and $\mathbf{t}_{\text{root}}$ -- translation to the GT root joint).
% }
% % \begin{tabular}{|c|c|l|r|r|r|}\hline
% \begin{tabular}{@{}clrrr@{}}\rowcolor{tablegray}\hline%\toprule
% \multicolumn{2}{c}{} & \multicolumn{3}{c}{Per joint position error (cm)} \\\cline{3-5}\rowcolor{tablegray}
% % \multicolumn{2}{r}{} 
% \multicolumn{2}{c}{\multirow{-2}{*}{\textsc{Human3.6M}}}
% & \multicolumn{1}{c|}{median} & \multicolumn{1}{c|}{mean} & \multicolumn{1}{c}{std.} \\\hline
% % \multirow{3}{*}{\rotatebox{90}{\footnotesize{Proposal}}} & 
% \multirow{4}{*}{\rotatebox{90}{ body }}
% & $\mathcal{B}, \mathbf{R}, \mathbf{t}_{\text{root}}$  & 4.572 & 5.715& 5.714 \\
% % & 
% & $\mathcal{B}, \mathbf{t}_{\text{root}}$  & 5.326 & 6.784& 7.019 \\
% % & 
% & $\mathbf{R}, \mathbf{t}_{\text{root}}$ & 5.066 & 6.037& 5.545 \\
% & $\mathbf{t}_{\text{root}}$ & 5.758 & 7.062& 6.830 \\
% \hline
% \end{tabular}
% \label{table:human36}
% \end{table}

